Practical Hash Functions for Similarity Estimation and Dimensionality Reduction

Hashing is a basic tool for dimensionality reduction employed in several aspects of machine learning. However, the perfomance analysis is often carried out under the abstract assumption that a truly random unit cost hash function is used, without concern for which concrete hash function is employed. The concrete hash function may work fine on sufficiently random input. The question is if it can be trusted in the real world when faced with more structured input. In this paper we focus on two prominent applications of hashing, namely similarity estimation with the one permutation hashing (OPH) scheme of Li et al. [NIPS'12] and feature hashing (FH) of Weinberger et al. [ICML'09], both of which have found numerous applications, i.e. in approximate near-neighbour search with LSH and large-scale classification with SVM. We consider mixed tabulation hashing of Dahlgaard et al.[FOCS'15] which was proved to perform like a truly random hash function in many applications, including OPH. Here we first show improved concentration bounds for FH with truly random hashing and then argue that mixed tabulation performs similar for sparse input. Our main contribution, however, is an experimental comparison of different hashing schemes when used inside FH, OPH, and LSH. We find that mixed tabulation hashing is almost as fast as the multiply-mod-prime scheme ax+b mod p. Mutiply-mod-prime is guaranteed to work well on sufficiently random data, but we demonstrate that in the above applications, it can lead to bias and poor concentration on both real-world and synthetic data. We also compare with the popular MurmurHash3, which has no proven guarantees. Mixed tabulation and MurmurHash3 both perform similar to truly random hashing in our experiments. However, mixed tabulation is 40% faster than MurmurHash3, and it has the proven guarantee of good performance on all possible input.

==> hashing.tex <==
\section{Similarity estimation with practical hash functions}
\label{sec:hashing}
In this paper we perform experiments comparing several families of hash
functions. We
give a quick description of these below. We also discuss the hash functions'
merits in relation to similarity estimation and present an experimental
comparison of evaluation times.

We say that a family $\mathcal{H}$ of hash
functions $h : U\to [m]$ is $t$-wise independent (or just $t$-independent) if,
for any set $S\subseteq U$ with
$|S|=t$, the keys of $S$ hash uniformly and independent of each other when $h$
is chosen uniformly at random from $\mathcal{H}$. We say that $\mathcal{H}$ is
universal, if for any two distinct keys $x,y\in U$ we have $\Prp{h(x) = h(y)}
\le 1/m$ over the choice of $h$.

\paragraph{Polynomial hashing}
The perhaps most classic hashing scheme we know dates back to Carter and
Wegman \cite{CarterW79} and is taught in undergrad algorithms courses all
over the world using \cite{clrs}. Fix some prime $p \ge m$. To get at
$t$-independent hash function $h : [p]\to [m]$ we choose $t$
integers, $a_0,\ldots, a_{t-1}$, uniformly at random from $[p]$ and define
\[
    h(x) = ((a_0 + a_1\cdot x + \ldots + a_{t-1}\cdot x^{t-1}) \bmod p)
    \bmod m\ .
\]
To efficiently implement this we may pick $p = 2^q-1$ a Mersenne prime and use
that
\[
    x\equiv x \bmod 2^q + \floor{x/2^q} \mod p\ .
\]
However, even then if we want to hash into $[2^{32}]$ we must pick $q\ge 61$
and evaluating $h$ then requires evaluating several 128-bit multiplications
which may be very slow compared to other hash functions.

Throughout the paper we will denote a $t$-wise independent polynomial hash
function (degree $t-1$) by \emph{$t$-wise PolyHash}.

\paragraph{Multiply-shift hashing}
Multiply-shift hashing of Dietzfelbinger et al.~\cite{dietzfel97closest} is the
fastest universal hash family in the literature. To obtain a hash function $h :
[2^w] \to [m], m = 2^d$ we fix any
$\bar{w} \ge w+d-1$ and pick $a,b$ uniformly at
random from $[2^{\bar{w}}]$. We then define
\[
    h(x) = \floor{(a\cdot x + b \bmod 2^{\bar{w}})/2^{\bar{w}-d}}\ .
\]
In particular, if we want $h$ to take 32-bit integers and produce 32-bit
integers we may pick $\bar{w} = 2^{64}$, choose $a,b$ as random 64-bit integers
and implement $h$ using a simple multiplication, addition and shift as follows:
\begin{verbatim}
h(x) = (a*x+b) >> 32
\end{verbatim}

\paragraph{Mixed tabulation}
Mixed tabulation was introduced by Dahlgaard, et al.~\cite{DahlgaardKRT15} to
provide an efficient hash function with very strong theoretical guarantees such
as uniform hashing for fixed sets and low bias when used with one permutation
hashing. For simplicity assume that we are hashing from the universe $[2^w]$
and fix integers $c,d$ such that $c$ is a divisor of $w$. Tabulation-based
hashing views each key $x$ as a list of $c$ characters $x_0,\ldots, x_{c-1}$,
where $x_i$ consists of the $i$th $w/c$ bits of $x$. We say that the alphabet
$\Sigma = [2^{w/c}]$. Mixed tabulation uses $x$ to derive $d$ additional
characters from $\Sigma$. To do this we choose  $c$ tables $T_{1,i} : \Sigma\to
\Sigma^d$ uniformly at random and let $y = \oplus_{i=0\ldots c} T_{1,i}[x_i]$
(here $\oplus$ denotes the XOR operation). The $d$ derived characters
are then $y_0,\ldots , y_{d-1}$. To create the final hash value we additionally
choose $c+d$ random tables $T_{2,i} : \Sigma\to [m]$, where $[m]$ is the
output range. The final hash value is then
\[
    h(x) = \bigoplus_{i\in [c]} T_{2,i}[x_i] \bigoplus_{i\in [d]}
    T_{2,i+c}[y_i]\ .
\]
The key to mixed tabulations efficiency is that all operations can be
implemented very fast due to the word-parallelism of the XOR operation and the
small table sizes. As an example if we wish to hash 32-bit values using $4$
characters each table has size $2^{32/4} = 256$ and easily fits in fast
cache. We may implement $h$ with $c=d=4$ and 32-bit keys and values as follows:
\begin{verbatim}
uint64_t mt_T1[256][4];
uint32_t mt_T2[256][4];

uint32_t mixedtab(uint32_t x) {
  uint64_t h=0; // Final hash value
  for(int i = 0;i < 4;++i, x >>= 8)
    h ^= mt_T1[(uint8_t)x][i];
  uint32_t drv=h >> 32;
  for(int i = 0;i < 4;++i, drv >>= 8)
    h ^= mt_T2[(uint8_t)drv][i];
  return (uint32_t)h;
}
\end{verbatim}

The main drawback to mixed tabulation hashing is that it needs a relatively
large random seed to fill out the tables $T_1$ and $T_2$. However, as noted in
\cite{DahlgaardKRT15} for all the applications we consider here it suffices to
fill in the tables using a $\Theta(\log |U|)$-independent hash function.

\subsection{Relation to similarity estimation}
While hashing provides very efficient solutions to similarity estimation one
must be careful to use a hash function with the right guarantees.
For one permutation hashing, both \cite{li12oneperm} and
\cite{Shrivastava14oneperm} suggest using polynomial hashing of
Carter and Wegman~\cite{CarterW79} as described above. However, we know from
\cite{PatrascuT16} that estimating the Jaccard similarity with small bias using
MinHash requires large independence. In particular if we want bias inversely
polynomial in $|U|$ we need $\Omega(\log |U|)$-independence. With polynomial
hashing this requires us to evaluate a $\Omega(\log |U|)$-degree polynomial
which is very slow (see comparison below). Meanwhile, this kind of polynomially
small bias can be obtained by Twisted tabulation
\cite{PT13:twist,dahlgaard14minwise} which can be seen as weaker variant of
mixed tabulation.
Trying to get around this limitation of minwise hashing was previously studied
in \cite{dahlgaard13nnbottomk} for large-scale learning based on bottom-$k$
sketches \cite{broder97onthe,thorup13bottomk}, however they only compared with
a nearest neighbour classifier which was impractical for large training sets.

While we know that MinHash can be done with $O(\log |U|)$-independence (see
\cite{Indyk01}) it is not even clear if this suffices for one permutation
hashing. However, it was shown in \cite{DahlgaardKRT15} that if we use mixed
tabulation for one permutation hashing, then we can estimate the Jaccard
similarity ``essentially as well'' as with truly random hash functions (i.e.
with a small bias inversely polynomial in $|U|$).

%The authors of \cite{Shrivastava14oneperm} also mention Nisan's PRG
%(which we have already discussed) and the result of \cite{mitzenmacher08hash},
%which states that simple $2$-independent hash
%functions suffice for most applications if the input has sufficient entropy.
%However, in most contexts, we actually seek to exploit highly structured
%data to obtain efficient classifiers or search structures, and clearly this
%result is not useful in such applications. Indeed, our experiments confirm that
%these hash functions may yield large bias in practice.

Table~\ref{tab:times} compares the running of the different hash
functions. As we can see mixed tabulation is roughly three times slower than
multiply-shift but almost twice as fast as a $2$-wise PolyHash function. This
is likely due to the involvement of 128-bit multiplication
and modulo, which are very costly operations. We have chosen a $20$-wise
PolyHash function to represent roughly $\Theta(\log |U|)$-independence. As can
be seen this function is more than 20 times slower than mixed tabulation.
32-bit keys and output values were chosen for convenience to enable fast
implementation of multiply-shift hashing and polynomial hashing (which would
otherwise require 256-bit multiplications).



==> proof.tex <==
\section{Why Simple Hash Functions Fail}
\label{sec:proof}
Next, we prove that simple hash functions such as
multiply-shift~\cite{dietzfel97closest} and $2$-independent polynomial hashing
(from here, 2-wise PolyHash)~\cite{CarterW79} ``fail'' on structured inputs.
We note that it is outside the scope of this paper to provide bad inputs
for every hash family used in practice, and we thus focus on these very widely
used families.

For some intuition on the problem, consider the following input: Let $A$ and
$B$ be two sets such that $A\cap B = \{0,1,\ldots, n-1\}$ for some $n$ and
their symmetric difference is $n$ randomly chosen distinct integers
greater than $n$. We then have $J(A,B) = \frac{n}{2n} = 1/2$. If we consider
the polynomial hash function $h(x) = ax+b \bmod p$ we observe that when
hashing consecutive keys, e.g. $A \cap B$, there are roughly two cases
depending on $a$. Either the hash values will generate ``clusters'' of
consecutive hash values as illustrated in Figure~\ref{fig:wheel}, or the hash
values will be very evenly spread out. This behaviour is very bad for minwise
hashing as it leads to highly biased estimates; If the hash values are
clustered as in Figure~\ref{fig:wheel} most of the bins will contain a smallest
element from the symmetric difference of $A$ and $B$, and if the the hash
values are very evenly spread out most of the bins will contain a smallest
element from $A \cap B$.
\begin{figure}[ht]
\begin{center}
\includegraphics[width=.25\textwidth]{figures/wheel.pdf}
\caption{Illustration of hashing consecutive keys with $h(x) = ax+b\bmod p$.
The circles correspond to consecutive keys and the squares to keys with random
values.}
\label{fig:wheel}
\end{center}
\end{figure}

We show two theorems. Theorem \ref{thm:evenlySplit} shows that $h$ is likely to
give hash values to the keys of $A \cap B$ that are very evenly split. In
contrast this happens with exponentially low probability when the hash values
are distributed using a truly random hash function.
Theorem~\ref{thm:concentrated} shows that with a non-negligible probability,
$h$ gives hash values to the keys of $A\cap B$ that are very clustered (i.e. as
in Figure~\ref{fig:wheel}). In contrast this almost never happens with truly
rnadom hash functions. The proofs are omitted due to space constraints.
\begin{theorem}
	\label{thm:evenlySplit}
	With probability $> \frac{1}{2}$ it holds that:
	every pair of hash values $h(x),h(y)$
	with $x,y \in A \cap B$ differ by at least $\frac{p}{4n}$. If we instead
	hashed using a truly random hash function this would happen with
	probability	$\le 2^{-\Omega(n)}$.
\end{theorem}

\begin{theorem}
	\label{thm:concentrated}
	For any $\eps > 0$ it holds with probability $\Omega(\eps)$ that:
	there exists $\Omega(n)$ disjoint pairs $x,y \in A \cap B$ such
	that the hash values $h(x),h(y)$ differ by at most $\frac{\eps p}{n}$.
	If we instead hashed using a truly random hash function this would happen
    with probability $\le \eps^{\Omega(n)}$.\sdtodo{We don't have a proof for
    this.}
\end{theorem}

